Nonparametric Composite Hypothesis Testing in an Asymptotic Regime

We investigate the nonparametric, composite hypothesis testing problem for arbitrary unknown distributions in the asymptotic regime where both the sample size and the number of hypotheses grow exponentially large. Such asymptotic analysis is important in many practical problems, where the number of variations that can exist within a family of distributions can be countably infinite. We introduce the notion of \emph{discrimination capacity}, which captures the largest exponential growth rate of the number of hypotheses relative to the sample size so that there exists a test with asymptotically vanishing probability of error. Our approach is based on various distributional distance metrics in order to incorporate the generative model of the data. We provide analyses of the error exponent using the maximum mean discrepancy (MMD) and Kolmogorov-Smirnov (KS) distance and characterize the corresponding discrimination rates, i.e., lower bounds on the discrimination capacity, for these tests. Finally, an upper bound on the discrimination capacity based on Fano's inequality is developed. Numerical results are presented to validate the theoretical results.

==> composite.tex <==
\section{Supervised Learning with Distinct Distributions} 

{\color{red} This section should be removed?} {\color{blue} Perhaps not? Or, we can merge all the results with composite and distinct distributions into one section as Analysis Results.}

{\color{red} Yes, please combine results for composite and distinct distributions into one section. Essentially, result for distinct distribution can follow as a special case of composite distribution.}



==> idevn.tex <==
% ITRANS Devanagari Header for TeX/LaTeX.
% using either Devnac or Devnag font
% Defines devanagari fonts in various sizes
% Also includes some macros for the ITRANS song book....
%-----
% Copy this file to someplace where TeX can find it, the best place
% is usually the ITRANS lib/ directory. Make sure to add that directory
% to the TEXINPUTS environment variable.
%-----
% created: avinash chopde, february 1994
%          avinash@aczoom.com
% modified: may 2001, 2007, 2009.
% Apr 2007: use of \fransdvng, \Largedvng, etc caused an extra space to
% be added after those commands - need to put % comment start after
% magstep1, etc in \Largedvng, etc definitions
% ----
% 2009:
% The current TeX distribution, texlive, has latest Velthuis Devnag
% package which does not have j~n, and also removes old \char43.
% The "dvnb" font has j~n at 224 and 236. So, updated all tex files
% to refer to dvnb10 instead of dvng10 (though kept names \largedvng, etc
% the same), and change ja-nya and gya in dvng and dvngfull IFM files
% to refer to 224/236.
% ----
% $Header:$
% -----------------------------------------------------------------
%% Usage:
%% Include this file somewhere in the beginning of your input file.
% \input <thisfilename>
%% Then, if you are using Frans's font, add these lines (uncommented):
% #indianifm=dvng_is.ifm  % ITRANS command
% #indianfont=\fransdvnb
%% If you are using the PostScript Devnac font that came with ITRANS, add
%% these lines (uncommented):
% #indianifm=dvnc.ifm  % ITRANS command
% #indianfont=\postdvng
%% Then, whenever you need to use some particular size of the font,
%% use the following command:
% \let\usedvng=\largedvng % usedvng is used by \fransdvng or \postdvng
%% sizes available: normaldvng < largedvng < LARGEdvng < hugedvng
% see the file ../doc/sample.itx for an example.
% -----------------------------------------------------------------
\newif\iffrans
% -----------------------------------------------------------------
% Page commands (for LaTeX ONLY, use one of these commands in preamble)
\def\portraitpage{%
    \setlength{\topmargin}{-0.50in} % real margin == this + 1in
    \setlength{\oddsidemargin}{-0.0in} % real margin == this + 1in
    \setlength{\evensidemargin}{-0.0in} % real margin == this + 1in
    \setlength{\columnsep}{20pt}
    \setlength{\columnseprule}{0.4pt}

    % Use Portrait Size Page
    \setlength{\textwidth}{6.5in}
    \setlength{\textheight}{9.0in}%
}
\def\landscapepage{%
    \typeout{Landscape Mode: be sure to print in landscape format}
    \typeout{   (for dvips, use -t landscape option)}
    
    \setlength{\topmargin}{-0.75in} % real margin == this + 1in
    \setlength{\oddsidemargin}{-0.0in} % real margin == this + 1in
    \setlength{\evensidemargin}{-0.0in} % real margin == this + 1in
    \setlength{\columnsep}{20pt}
    \setlength{\columnseprule}{0.4pt}

    % Use Landscape Size Page
    \setlength{\textwidth}{9.5in}
    \setlength{\textheight}{7in}%
}
% -----------------------------------------------------------------
% Font Stuff
\font\sixrm=cmr6
\font\sevenrm=cmr7
\font\eightrm=cmr8
\font\ninerm=cmr9
\font\tenrm=cmr10

\let\smallcmr=\sixrm
\let\titlefont=\eightrm

\def\devnmode{
    \tolerance=10000
    \pretolerance=10000
    \normalbaselines
    \hyphenchar\devnfont=-1 % do not hyphenate words using this font
	%
	% If using Frans's font, need to make punctuation chars active.
	\iffrans
	    \specialsforfrans % turn this on for Frans' font only.
	\fi
    % \englfont % default font is english font.
    \devnfont % default font is devanagari font.
}
% ------------------------------------------------------------------------
% Devanagari font macros
% sizes: normal < large < Large < LARGE < huge < Huge
% Apr 2007: careful with multi-line commands - add % immediately after
% magstep, or when using font at 12pt etc to swallow up newline, etc

% 10pt text
\def\normaldvng{
    \iffrans
        \font\devnfont=dvnb10
        \font\englfont=cmr10
    \else
        \font\devnfont=dnh at 12pt% size looks like 10pt
        \font\englfont=cmbx10
    \fi
    \normalbaselineskip=15pt\devnmode}

% 10.95pt text
\def\largedvng{\iffrans \font\devnfont=dvnb10 scaled\magstephalf%
          \font\englfont=cmr10 scaled\magstephalf%
    \else \font\devnfont=dnh at 14pt% size looks like 11pt
          \font\englfont=cmbx10 scaled\magstephalf%
    \fi
    \normalbaselineskip=16pt\devnmode}

% 12pt text
\def\Largedvng{\iffrans \font\devnfont=dvnb10 scaled\magstep1%
          \font\englfont=cmr10 scaled\magstep1%
    \else \font\devnfont=dnh at 16pt% size looks like 12pt
          \font\englfont=cmbx10 scaled\magstep1%
    \fi
    \normalbaselineskip=18pt\devnmode}

% 14.4pt text
\def\LARGEdvng{\iffrans \font\devnfont=dvnb10 scaled\magstep2% 14.4pt
          \font\englfont=cmr10 scaled\magstep2%
    \else \font\devnfont=dnh at 19pt% size looks like 14.4 pt
          \font\englfont=cmbx10 scaled\magstep2%
    \fi
    \normalbaselineskip=21pt minus2pt\devnmode}

% 17.28pt text
\def\hugedvng{\iffrans \font\devnfont=dvnb10 scaled\magstep3% 17.28pt
          \font\englfont=cmr10 scaled\magstep3%
    \else \font\devnfont=dnh at 22pt% size looks like 17.28 pt
          \font\englfont=cmbx10 scaled\magstep3%
    \fi
    \normalbaselineskip=25pt\devnmode}

% 20.74pt text
\def\Hugedvng{\iffrans \font\devnfont=dvnb10 scaled\magstep4% 20.74
          \font\englfont=cmr10 scaled\magstep4%
    \else \font\devnfont=dnh at 25pt% size looks like 20.74 pt
          \font\englfont=cmbx10 scaled\magstep4%
    \fi
    \normalbaselineskip=28pt\devnmode}

% ------------------------------------------------------------------------
% (Must do \let\usedvng after normaldvng is defined...)
%
\let\usedvng=\normaldvng	% default font size definition

\def\fransdvng{\franstrue\usedvng}

\def\postdvng{\fransfalse\usedvng}

% ------------------------------------------------------------------------
% Macro for song listings (verbatim mode---see page 381 of the TeXbook)
\def\obeyspaceslines{\def\par{\leavevmode\null\endgraf\penalty-500\relax}%
                        \obeylines \obeyspaces}
% actually, the TeXbook defn has problems -- according to comp.text.tex
% readers, I needed to add the \null and \relax above to make it correct!
% otherwise TeX will eat up any number that starts a line!!!!!
%{\obeyspaces\global\let =\ } % TeX sets space = "\space", change it to "\ "
{\obeyspaces\global\let =~} % use this for a non-breaking space

\def\threedots{{\englfont%
    \leavevmode\hbox{\hskip2pt .\hskip2pt .\hskip2pt .\hskip2pt}}}

% For Frans's devanagari font, make punctuation chars that are absent from
% the font active characters, and define them to use the roman font punctuation.
% These characters have to be made special
% NO NEED TO DO THIS FOR THE PostScript Devnac font...
\def\specialsforfrans{%
	\catcode`\(=\active
	\catcode`\,=\active
	\catcode`\)=\active
	\catcode`\:=\active
	\catcode`\;=\active
	\catcode`\!=\active
	\catcode`\?=\active
	\catcode`\'=\active
	\catcode`\"=\active
	\catcode`\/=\active
	\catcode`\|=\active%
}
% define the commands for the punctuations
{\specialsforfrans
	\gdef,{{\englfont\char`\,}}
	\gdef({{\englfont\char`\(}}
	\gdef){{\englfont\char`\)}}
	\gdef:{{\englfont\char`\:}}
	\gdef;{{\englfont\char`\;}}
	\gdef!{{\englfont\char`\!}}
	\gdef?{{\englfont\char`\?}}
	\gdef'{{\englfont\char`\'}}
	\gdef"{{\englfont\char`\"}}
	\gdef/{{\englfont\char`\/}}
	\gdef|{.}
	% CANNOT do the same for - (numbers like kern-0.3 get screwed up!)
	% \catcode`\-=\active % NOTE: this implies that minus cannot be used (no numbers)!
	% \def-{{\englfont\char`\-}} % DONT EVER TURN THIS ON!
	% Therefore, have to use \- in the input song
	% Similarly, cannot use . in input text (to get roman period)
	% Use \. instead.
}
% Frans's Font does not have -, but cannot make - an active character,
% so you must use \- to get a dash (same goes for . (dot) use \. instead).
% For PostScript out, the hdr.ips defines a \- procedure, so all works
% there too..... (IF your PostScript intepretor accepts \ in a name!)
% See the comments regarding "specialsforfrans" in this file to see how
% other punctuation characters are handled for Frans's devnag font...
% ------------------
%
% ------ definitions for song headings, etc ------
\def\fileinfo{%
    \ifx\songfile\undefined % songfile is defined when multiple
    			    % .s files are combined by "isongcat" program.
        \ifx\jobname\undefined
            \rightline{\hbox to 120pt{\hfill\smallcmr ITRANS Song Book}}%
	\else
            \rightline{\hbox to 120pt{\smallcmr ITRANS Song Book:\hfill{\jobname}.s}}%
	\fi
    \else
        \rightline{\hbox to 120pt{\smallcmr ITRANS Song Book:\hfill{\songfile}}}%
    \fi
}

% songtitle - use if needed. Invoke this after a \startsong statement
% Assumes that both \startsong and \songtitle lines in the input text
% do not contain a % at the end....
    \def\stitle#1{}	% unused today...
    \def\film#1{\def\vvfilm{#1}}
    \def\starring#1{}
    \def\singer#1{\def\vvsinger{#1}}
    \def\lyrics#1{\def\vvlyrics{#1}}
    \def\music#1{\def\vvmusic{#1}}

    \def\printtitle{{% print out vvfilm, vvsinger, vvlyrics, vvmusic
	\ifx\vvfilm\undefined \def\vvfilm{} \fi
	\ifx\vvsinger\undefined \def\vvsinger{} \fi
	\ifx\vvlyrics\undefined \def\vvlyrics{} \fi
	\ifx\vvmusic\undefined \def\vvmusic{} \fi
	\vskip3pt
	\baselineskip=0pt% local def only, using 2 {'s to define \printtitle..
	%
	% Now, print out legend only if atleast one of the args is non-{}
	\def\vvnonempty{1} % initialize non-empty to TRUE
	\ifx\vvfilm\empty \else\def\vvnonempty{0}\fi % check film non-empty
	\ifx\vvsinger\empty \else\def\vvnonempty{0}\fi % check singers
	\ifx\vvlyrics\empty \else\def\vvnonempty{0}\fi % check lyrics
	\ifx\vvmusic\empty \else\def\vvnonempty{0}\fi % check music
	% if any args present, print out legend:
	\nobreak
	\if0\vvnonempty
	    \setbox0=\hbox{\titlefont {\smallcmr film:} \vvfilm%
	    			   \quad{\smallcmr singer:} \vvsinger%
				   \quad{\smallcmr lyrics:} \vvlyrics%
				   \quad{\smallcmr music:} \vvmusic}%
	    \ifdim\wd0>\hsize
		% too large, split into two lines
		\hbox to\hsize{\titlefont {\smallcmr film:} \vvfilm%
	    			   \quad{\smallcmr singer:} \vvsinger\hfill}%
		\vskip2pt
		\hbox to\hsize{\titlefont {\smallcmr lyrics:} \vvlyrics%
				   \quad{\smallcmr music:} \vvmusic\hfill}%
	    \else
		\hbox to\hsize{\titlefont {\smallcmr film:} \vvfilm%
	    			   \hfill{\smallcmr singer:} \vvsinger%
				   \hfill{\smallcmr lyrics:} \vvlyrics%
				   \hfill{\smallcmr music:} \vvmusic\hfill}%
	    \fi
	\fi
	\nobreak
	}}% printtitle

% ------------------------------------------------
%%%%%%%%%%%%% Shrisha Rao's macros %%%%%%%%%%%%%%
\def\ldq{{\englfont ``\hskip+0.1em}} % Avinash Chopde's definitions
\def\rdq{{\englfont ''}}           % to make quotes possible.

\def\ast{{\englfont *}}      % defined to use an asterisk
\def\dash{{\englfont ---}}   % defined to use a long dash
\def\spl{{\englfont \S}}     % defined to use a special symbol

\def\lsq{{\englfont `\hskip+0.1em}}  % single open-quote
\def\rsq{{\englfont '}}            % single close-quote

\def\?{{\englfont ?}}        % defined to use a question-mark
%%%%%%%%%%%%% End of Shrisha Rao's macros %%%%%%%%%%%%%%
% ------------------------------------------------

\def\startsong{\bgroup 
	\def\-{{\englfont -}}%
	\def\.{{\englfont .}}%
	\usedvng % use whatever font the user wants...default normaldvng
	\englfont % usedvng makes default font indian, restore english font
	\parindent=7pt%
        \obeyspaceslines}

\def\endsong{%
	\nobreak
	\vskip 9pt plus1fill % fill this page if no more material available
	\fileinfo\smallskip
	\hrule height0.4pt%
	\egroup
	}

% ----------------------- End of idevn.tex ------------------------

